Evolving R2 to R2+: Optimal, Delayed Line-of-sight Vector-based Path Planning

A vector-based any-angle path planner, R2, is evolved in to R2+ in this paper. By delaying line-of-sight, R2 and R2+ search times are largely unaffected by the distance between the start and goal points, but are exponential in the worst case with respect to the number of collisions during searches. To improve search times, additional discarding conditions in the overlap rule are introduced in R2+. In addition, R2+ resolves interminable chases in R2 by replacing ad hoc points with limited occupied-sector traces from target nodes, and simplifies R2 by employing new abstract structures and ensuring target progression during a trace. R2+ preserves the speed of R2 when paths are expected to detour around few obstacles, and searches significantly faster than R2 in maps with many disjoint obstacles.

==> __fig_phantom.tex <==
\tikzset{
    pics/phantom/.style n args={0}{ code={ 
        \path (\ul, 0) coordinate (xsrc);
        \path (15*\ul, 3*\u) coordinate (xtgt);
    
        % second collision obs
        \fill [swatch_obs] 
            (2*\ul, 3*\ul) coordinate (xb4) -- ++(90:4*\ul) coordinate (xb5) -- ++(0:\ul) -- ++(90:-2*\ul) -- ++(0:3*\ul) -- ++(90:-2*\ul) 
            -- ++(0:6*\ul) -- ++(90:-\ul) -- ++(0:-7*\ul) -- ++(90:2*\ul) coordinate (xb1) -- ++(0:-2*\ul) coordinate (xb2) -- ++(90:-\ul) coordinate (xb3);
    
        % first collision obs
        \fill [swatch_obs] 
            (7*\ul, 6*\ul) coordinate (x10) -- ++(90:2*\ul) coordinate (x11) -- ++(0:\ul) coordinate (x12) -- ++(90:-\ul) -- ++(0:6*\ul) -- ++(90:-8*\ul) -- ++(0:-\ul) coordinate (xoom) -- ++(90:7*\ul) coordinate (x1) 
            -- ++(0:-\ul) coordinate (x2) -- ++(90:-\ul) coordinate (x3) -- ++(0:-\ul) coordinate (x4)  -- ++(90:\ul) coordinate (x5)
            -- ++(0:-\ul) coordinate (x6) -- ++(90:-2*\ul) coordinate (x7) -- ++(0:-\ul) coordinate (x8) -- ++(90:2*\ul) coordinate (x9);

    }},
}


\begin{figure}[!ht]
\centering
\subfloat[\label{fig:phantoma} ] {%
    \begin{minipage}[b]{8cm}
    \centering
    \begin{tikzpicture}[]
        \clip (-\u, -\u) rectangle ++(16*\ul, 9*\ul);
        \pic at (0,0) {phantom};

        % cast from src to tgt and collision
        \draw [dotted] (xsrc) -- (xtgt)
            coordinate [pos=12/14] (xcol) {};
        \node [cross pt] at (xcol) {};
        
        % src link, node and obs
        \node (nsrc) [svy pt={left, yshift=1mm}{$\mx_S$}] at (xsrc) {};
        \draw [sxlink] (nsrc) -- ++(0:-2*\ul);
        
        % tgt link and node 
        \node (ntgt) [tvu pt={below left, yshift=-1mm, xshift=1mm}{$\mx_T$}] at (xtgt) {};
        \draw [txlink] (ntgt) -- ++(90:-3*\ul);
    
        % first trace's nodes
        \draw [trace] (xcol) -- (x1) -- (x2) -- (x3) -- (x4) -- (x5) -- (x6) -- (x7) -- (x8) -- (x9) -- (x10) -- (x11) -- (x12) -- ++(90:-\u);
        \node (n1 tph) [tph pt={right}{$\mx_1$}] at (x1) {};
        \pic at (x12) {trace grp={right}{0:$\mx_3$}{n12 strtm}{n12 ttrtm}};
        % \node [separate={right, xshift=2mm, yshift=-1mm}{$\mx_3$}] at (x12) {};
        % \node (n12 strtm) [trtm pt, xshift=-\uss] at (x12) {};
        % \node (n12 ttrtm) [trtm pt, xshift=\uss] at (x12) {};
    
        % paths
        \draw [tlink] (n12 ttrtm) edge (n1 tph) (n1 tph) edge (ntgt);
        \draw [slink] (n12 strtm) edge (nsrc);
    \end{tikzpicture}
    \end{minipage}
} \\
\subfloat[\label{fig:phantomb}] {%
    \begin{minipage}[b]{8cm}
    \centering
    \begin{tikzpicture}[]
        \clip (-\u, -\u) rectangle ++(16*\ul, 9*\ul);
        \pic at (0,0) {phantom};
        
        % draw a line from xb5 to x1 to show pruning
        \draw [dotted] (xb5) -- (x1);
        
        % cast from src to x10 and collision
        \draw [dotted] (xsrc) -- (x10)
            coordinate [pos=4/6] (xcol2) {};
        \node [cross pt] at (xcol2) {};
        
        % src link, node and obs
        \node (nsrc) [svy pt={left, yshift=1mm}{$\mx_S$}] at (xsrc) {};
        \draw [sxlink] (nsrc) -- ++(0:-2*\ul);
        
        % tgt link and node 
        \node (ntgt) [tvu pt={below left, yshift=-1mm, xshift=1mm}{$\mx_T$}] at (xtgt) {};
        \draw [txlink] (ntgt) -- ++(90:-3*\ul);
    
        % first trace's nodes
        \node (n1 tph) [tph pt={right}{$\mx_1$}] at (x1) {};
        \node (n10 ttm) [ttm pt={below right, yshift=-1mm}{$\mx_2$}] at (x10) {};
        % \node [black pt={left}{$\mx_2$}] at (x8) {};

        % second trace's nodes
        \draw [trace2] (xcol2) -- (xb2) -- (xb3) -- (xb4) -- (xb5) -- ++(0:\u);
        % \node (nb2 tph) [tph pt={below right, yshift=-1mm}{$\mx_5$}] at (xb2) {};
        \pic at (xb5) {trace grp={left}{180:$\mx_4$}{nb5 strtm}{nb5 ttrtm}};
            
        % paths
        \draw [tlink] (nb5 ttrtm) edge (n10 ttm) (n10 ttm) edge (n1 tph) (n1 tph) edge (ntgt);
        \draw [slink] (nb5 strtm) edge (nsrc);
    \end{tikzpicture}
    \end{minipage}
}    
\caption{
Phantom points on a different best-hull are identified after a $\mntm$ node is pruned.
(a) Consider a trace that finds a phantom point at $\mx_1$, and the point becomes castable at $\mx_3$. 
Since the point is a target node of the trace (connected directly to the trace's trace-nodes), the trace will continue past $\mx_3$ instead of casting.
(b) Suppose the trace from (a) is interrupted by the interrupt rule, and a $\mntm$ node is placed at $\mx_2$.
A cast may subsequently be performed by the overlap rule from $\mx_S$ to the $\mntm$ node, which collides and causes a trace to reach $\mx_4$.
At $\mx_4$, the $\mntm$ node is pruned, exposing the phantom point at $\mx_1$.
As the $\mntm$ node is placed by an earlier incomplete trace, the phantom point can be inferred  to lie on a different best-hull. 
By converting the point to a $\mntm$ node, the point becomes castable, and casts can occur between different best-hulls.
}
\label{fig:phantom}
\end{figure}


%%%%%%%%%%%%%%% draft 1 %%%%%%%%%%%%%%%%%%%%%
% \fill [swatch_obs] 
%     (0, 0) -- ++(90:5*\ul) -- ++(0:12*\ul) -- ++(90:-\ul) -- ++(0:-11*\ul) coordinate (x1) -- ++(90:-4*\ul) coordinate (x2);
% \fill [swatch_obs]
%     (3*\ul, 0) -- ++(90:3*\ul) -- ++(0:4*\ul) coordinate (x4) -- ++(90:-\ul) coordinate (x3b) -- ++(0:-3*\ul) coordinate (x3) -- ++(90:-\ul) coordinate (x2b) -- ++(0:7*\ul) coordinate (xsrc) -- ++(90:-\ul);

% \node (ntgt) [tvu pt={right}{$\mx_T$}] at (10*\ul, 6*\ul) {};
% \node (nsrc) [svu pt={right}{$\mx_S$}] at (xsrc) {};
% \draw [txlink] (ntgt) -- ++(90:\ul);
% \draw [sxlink] (nsrc) -- ++(90:-2*\ul);
% \draw [dotted] (nsrc) -- (ntgt) 
%     node (xcol) [coordinate, pos=3/5] {};
% \draw [trace] (xcol) -- (x1) -- (x2) -- ++(0:-\u);
% \draw [trace2] (nsrc) -- (x2b) -- (x3) -- (x3b) -- (x4) -- ++(0:-\u);
% \node (ncol) [cross pt] at (xcol) {};

% \node (n1 tph) [tph pt={left}{$\mx_1$}] at (x1) {};
% \node (n2 ttm) [ttm pt={below right, xshift=1mm}{$\mx_2$}] at (x2) {};
% \node (n3 tph) [tph pt={left}{$\mx_3$}] at (x3) {};
% \node [separate={right, xshift=2mm}{$\mx_4$}] at (x4) {};
% \node (n4 strtm) [trtm pt, xshift=\uss] at (x4) {};
% \node (n4 ttrtm) [trtm pt, xshift=-\uss] at (x4) {};

% \draw [slink] (n4 strtm) edge (nsrc);
% \draw [tlink] (n4 ttrtm) edge (n3 tph) (n3 tph) edge (n2 ttm) (n2 ttm) edge (n1 tph) (n1 tph) edge (ntgt);
%%%%%%%%%%%%%%% draft 1 %%%%%%%%%%%%%%%%%%%%%

==> sym_ph.tex <==
\raisebox{0pt}{
    \tikz{
        \clip (-1.1mm, -1.1mm) rectangle ++(2.2mm, 2.2mm);
        \node [ph pt={}{}{}] at (0,0) {};
    }
}
